An Abstract Approach to Stratification in Linear Logic

We study the notion of stratification, as used in subsystems of linear logic with low complexity bounds on the cut-elimination procedure (the so-called light logics), from an abstract point of view, introducing a logical system in which stratification is handled by a separate modality. This modality, which is a generalization of the paragraph modality of Girard's light linear logic, arises from a general categorical construction applicable to all models of linear logic. We thus learn that stratification may be formulated independently of exponential modalities; when it is forced to be connected to exponential modalities, it yields interesting complexity properties. In particular, from our analysis stem three alternative reformulations of Baillot and Mazza's linear logic by levels: one geometric, one interactive, and one semantic.

==> CohSwap.tex <==
Recalling \refdef{SwapSens}, we need to prove that, in the coherence space model, for every cut-free, $\eta$-expanded linear logic \dr\ $\pi$,
$$\pi'\swapping\pi\textrm{ implies }\cX(\pi')\neq\cX(\pi),$$
where the relation $\swapping$ is defined in \refdef{Swapping}, and $\cX$ is the functor introduced at the beginning of \refsect{Completeness}, just before \refprop{Factoring}. We recall the definitions here for convenience:
\begin{itemize}
	\item $\pi'\swapping\pi$ means that $\pi'$ is obtained by replacing a non-null number of subnets of the form $\id_{X\ltens X}$ of $\pi$ with the net $\gamma_{X,X}$; these two nets are given in \reffig{IdAndFlip}.
	\item $\cX$ is a functor from $\catPN$, the syntactic category of linear logic formulas and cut-free, $\eta$-expanded \dr s, to $\Coh$, the category of coherence spaces and linear functions. It is defined as the usual interpretation of formulas as coherence spaces and proofs as linear functions (or cliques), under the assignment mapping every propositional atom to a coherence space $\Xi$ such that $\id_{\Xi\ltens\Xi}\neq\gamma_{\Xi,\Xi}$, where $\id_{\Xi\ltens\Xi}$ is the identity of $\Xi\ltens\Xi$ and $\gamma_{\Xi,\Xi}$ is the function $\Xi\ltens\Xi\rightarrow\Xi\ltens\Xi$ ``swapping'' the two copies of $\Xi$.

	For instance, we can take $\Xi=\lone\lplus\lone$, where $\lone$ is the coherence space whose web is a singleton. In that case, the web of $\Xi$ has two elements $a,b$, and, seen as a clique, the morphism $\gamma_{\Xi,\Xi}$ is equal to
	$$\{((a,a),(a,a)),((a,b),(b,a)),((b,a),(a,b)),((b,b),(b,b))\},$$
	which is different from $\id_{\Xi\ltens\Xi}$, whose clique is $$\{((a,a),(a,a)),((a,b),(a,b)),((b,a),(b,a)),((b,b),(b,b))\}.$$
\end{itemize}

Then, we may restate swap-sensitivity for coherence spaces as follows: whenever we interpret propositional atoms with a space whose web has at least two elements, the semantics is able to tell apart a cut-free, $\eta$-expanded proof net $\pi$ from a proof net $\pi'$ obtained from $\pi$ by replacing at least one identity subnet (\reffig{IdAndFlip}, left) with a ``swap'' subnet (\reffig{IdAndFlip}, right).


==> Geometric.tex <==
\wip{Most proofs in this section are only sketched.}

\wip{The following definition does not work, but it's a start:}
\begin{defn}[Balanced path]
	\label{def:Balanced}
	\sloppy{Let $\pi$ a \MELL\ \ps. A \emph{path} of $\pi$ is a finite non-empty sequence of edges of $\pi$ such that two adjacent edges in the sequence have a link in common (so paths need not be directed or simple). The \emph{balance} of $\phi$, denoted by $\bal\phi$, is a relative integer defined by induction on the length of $\phi$:}
	\begin{itemize}
		\item if $\phi$ contains just one edge, $\bal\phi=0$;
		\item otherwise, let $e$ be the last edge of $\phi$, let $\phi'$ be the path obtained from $\phi$ by removing $e$, and let $e'$ be the last edge of $\phi'$. Then:
		\begin{itemize}
			\item if $e'$ is a premise (or the premise) of a \whynot\ or \ofcourse\ link $l$, and $e$ is the conclusion of $l$, then $\bal\phi=\bal{\phi'}+1$;
			\item if $e'$ is the conclusion of a \whynot\ or \ofcourse\ link $l$, and $e'$ is a premise (or the premise) of $l$, then $\bal\phi=\bal{\phi'}-1$;
			\item in all other cases, $\bal{\phi}=\bal{\phi'}$.
		\end{itemize}
	\end{itemize}
	A \emph{balanced path} is a path $\phi$ such that $\bal\phi=0$.
\end{defn}
\begin{proposition}
	Let $\pi$ be a net. Then, $\pi$ is weakly indexable iff all cycles in $\pi$ are balanced.
\end{proposition}
\begin{proof}
	Left to right is easy. Right to left is by induction on the size of $\pi$.\qed
\end{proof}
\begin{corollary}[Geometric characterization]
	Let $\pi$ be a proof net. Then, $\pi\in\MELLlev$ iff every cycle in the $\lpar$-closure of $\pi$ is balanced.
\end{corollary}
\begin{proof}
	Simply observe that weak indexability and indexability coincide on nets with at most one conclusion, and that a net is indexable iff its $\lpar$-closure is indexable.\qed
\end{proof}

In the case of cut-free \ps s, there is an even simpler characterization.
\begin{defn}[Balanced axiom in a cut-free \ps]
	\sloppy{Let $\pi$ be a cut-free \MELL\ \ps, and let $a$ be an \axiom\ link of $\pi$. If we take any one of its conclusions, and follow the directed path ``going down'' from it, the absence of \cut\ links guarantees us that such path ends in a unique conclusion of $\pi$. We call $\phi_1$ and $\phi_2$ the two paths determined in this way by the conclusions of $a$, and we say that $a$ is \emph{balanced} just if $\bal{\phi_1}=\bal{\phi_2}$.}
\end{defn}
\begin{prop}[Geometric characterization, cut-free case]
	\label{prop:AltDefCutFree}
	Let $\pi$ be a cut-free \MELL\ \ps. Then, $\pi\in\MELLlev$ iff every axiom of $\pi$ is balanced.
\end{prop}
\begin{proof}
	Assign $0$ to all conclusions of $\pi$, and ``go up''. This ``procedure'' deterministically assigns an index to all conclusions of axioms of $\pi$. Now, simply observe that axioms will be correctly indexed (\ie, both conclusions have the same index) iff every axiom of $\pi$ is balanced.\qed
\end{proof}


==> meLL.tex <==
\paragraph*{Formulas.}
The formulas of propositional unit-free multiplicative exponential linear logic (\MELL) are generated by the following grammar, where $X,X^\perp$ range over a denumerable set of propositional variables:
$$A,B::=X~|~X^\perp~|~A\ltens B~|~A\lpar B~|~\oc A~|~\wn A.$$
Linear negation is defined through De Morgan laws:
\begin{displaymath}
	\begin{array}{rclcrcl}
		(X)^\perp & = & X^\perp && (X^\perp)^\perp & = & X \\
		(A\ltens B)^\perp & = & A^\perp\lpar B^\perp && (A\lpar B)^\perp & = & A^\perp\ltens B^\perp \\
		(\oc A)^\perp & = & \wn A^\perp && (\wn A)^\perp & = & \oc A^\perp\\
		(\exists X.A)^\perp & = & \forall X.A^\perp && (\forall X.A)^\perp & = & \exists X.A^\perp \\
	\end{array}
\end{displaymath}
Two connectives exchanged by negation are said to be \emph{dual}. Observe that full propositional linear logic has a further pair of dual binary connectives, called \emph{additive} (denoted by $\&$ and $\oplus$). They are not strictly needed for our purposes, hence we restrict to \MELL\ in the paper.

Linear implication is defined as $A\llinimp B=A^\perp\lpar B$. Multisets of formulas will be ranged over by $\Gamma,\Delta,\ldots$

For technical reasons, it is also useful to consider \emph{\struct s}, which will be denoted by $\flat A$, where $A$ is a formula.

\paragraph*{Proofs.}
The proof theory of \MELL\ can be formulated using \pn s, originally introduced by \cite{Girard:LL,Girard:ProofNets}, and subsequently reformulated by other authors using alternative, but equivalent syntactical definitions. In this paper, we use a combination of the presentations given by \cite{DanosRegnier:PNHilb} and \cite{Tortora:AdditivesAndNormalizationI}, with a slight change in the terminology: the term ``proof structure'', introduced by~\cite{Girard:LL} and traditionally used in the literature, is here dismissed in favor of the term \emph{\ps}. On the contrary, the term \pn, i.e., a \ps\ satisfying certain structural conditions (the correctness criterion), retains its usual meaning.

\begin{figure}[t]
	\pict{links}
	\caption{Links.}
	\label{fig:Links}
\end{figure}
\begin{figure}[t]
	\pict{boxes}
	\caption{A box.}
	\label{fig:Boxes}
\end{figure}
In the following definition, and throughout the rest of the paper, unless explicitly stated we shall make no distinction between the concepts of \emph{formula} and \emph{occurrence of formula}. The same will be done for what we call \emph{links} and their occurrences.
\begin{defn}[\Ps]
	\label{def:Net}
	A \emph{\pps} is a pair $(\mathcal G,\mathsf B)$, where $\mathcal G$ is a finite graph-like object whose nodes are occurrences of what we call \emph{links}, and whose edges are directed and labelled by formulas or \struct s of \MELL; and $\mathsf B$ is a set of subgraphs of $\mathcal G$ called \emph{boxes}.
	\begin{itemize}
		\item Links (\reffig{Links}) are labelled by connectives of \MELL, or by one of the labels $\mathsf{ax}$, $\mathsf{cut}$, $\flat$, $\mathsf{pax}$. Two links labelled by dual connectives are said to be \emph{dual}. Each link has an arity and co-arity, which are resp.\ the number of its incoming and outgoing edges. The arity and co-arity is fixed for all links except \whynot\ links, which have co-arity $1$ and arbitrary arity. A nullary \whynot\ link is also referred to as a \weak\ link.
		
		\item The incoming edges of a link (and the formulas that label them) are referred to as its \emph{premises}, and are assumed to be ordered, with the exception of \cut\ and \whynot\ links; the outgoing edges of a link (and the formulas that label them) are referred to as its \emph{conclusions}.
		
		\item Premises and conclusions of links must respect a precise labeling (which depends on the link itself), given in \reffig{Links}. In particular, the edges labelled by \struct s can only be premises of \paxl\ and \whynot\ links;
		
		\item Each edge must be the conclusion of exactly one link, and the premise of at most one link. The edges that are not premises of any link (and the formulas that label them) are deemed \emph{conclusions} of the \pps. (Note that the presence of these ``pending'' edges, together with the fact that some premises are ordered, is why \pps s are not exactly graphs).
		
		\item A box is depicted as in \reffig{Boxes}, in which $\pi$ is a \pps, said to be \emph{contained} in the box. The links that are explicitly represented in \reffig{Boxes} (i.e., the \paxl\ links and the \ofcourse\ link) form the \emph{border} of the box. The unique \ofcourse\ link in the border is called the \emph{\pal} of the box, while the \paxl\ links are called \emph{\pax s}. We have the following conditions concerning boxes:
		\begin{enumerate}
			\item[a.] each \ofcourse\ link is the \pal\ of exactly one box;
			\item[b.] each \paxl\ link is in the border of exactly one box; 
			\item[c.] any two distinct boxes are either disjoint or included in one another.
		\end{enumerate}
	\end{itemize}
	
	A \emph{\ps} is a \pps\ having no \struct\ in its conclusions.
\end{defn}
\begin{defn}[Depth, size]
	\label{def:DepthSize}
	Let $\sigma$ be a \pps.
	\begin{itemize}
		\item A link (or edge) of $\sigma$ is said to have \emph{depth} $d$ if it is contained in $d$ (necessarily nested) boxes. The depth of a box of $\sigma$ is the depth of the links forming its border. The depth of a link $l$, edge $e$, or box $\cB$ are denoted resp.\ by $\Depth l$, $\Depth e$ and $\Depth\cB$. The depth of $\sigma$, denoted by $\Depth\sigma$, is the maximum depth of its links.
		\item The \emph{size} of $\sigma$, denoted by $\Size\sigma$, is the number of links contained in $\sigma$, excluding \pax s.
	\end{itemize}
\end{defn}
\begin{defn}[Switching]
	\label{def:Switching}
	Let $\sigma$ be a \pps. For each \parl\ link $l$ of $\sigma$, we define the set of \emph{jumps} of $l$, denoted by $J(l)$, as the set containing the links whose conclusions are the premises of~$l$. A \emph{switching} of $\sigma$ is an undirected graph built as follows:
	\begin{itemize}
		\item the conclusions of $\sigma$ are erased, and its edges considered as undirected;
		\item for each \parl\ link $l$, the premises of $l$ are erased, exactly one node $m\in J(l)$ is chosen and a new edge between $m$ and $l$ is added.
		\item the boxes at depth zero of $\sigma$ are collapsed into single nodes, i.e., if $\cB$ is a box at depth zero of $\sigma$, it is erased together with all the edges connecting its links to the rest of the structure, and replaced with a new node $l$; then, for any link $m$ of depth zero which was connected to a link of $\cB$, a new edge between $m$ and $l$ is added.
	\end{itemize}
\end{defn}
\begin{defn}[\Pn]
	\label{def:ProofNet}
	A \pps\ $(\mathcal G,\mathsf B)$ is \emph{correct} iff:
	\begin{itemize}
		\item all of its switchings are acyclic;
		\item for all $\cB\in\mathsf B$, the \pps\ contained in $\cB$ is correct.
	\end{itemize}
	A \emph{\pn} is a correct \ps.
\end{defn}
% With \pn s, we can give a notion of provability: a multiset of formulas $\Gamma$ is provable in \MELL\ iff there exists a \pn\ of conclusions $\Gamma$.

\paragraph*{Sequentiality.} We now introduce the notion of \emph{sequentializable} \ps, whose definition mimics the rules of a sequent calculus:
\begin{figure}[t]
	\pict{SPS}
	\caption{Rules for building sequentializable \ps s.}
	\label{fig:SPS}
\end{figure}
\begin{defn}[\Sps]
	\label{def:SeqNet}
	We define the set of \emph{\sps s} inductively: the empty \ps\ and the \ps\ consisting of a single \axiom\ link are sequentializable (daimon and axiom); the juxtaposition of two sequentializable \ps s is sequentializable (mix); if $\sigma$, $\sigma_1$, $\sigma_2$ are \sps s of suitable conclusions, the \ps s of \reffig{SPS} are sequentializable; if
	\pict{PromotionSPS1}
	is a \sps, then the \ps
	\pict{PromotionSPS2}
	is sequentializable (promotion); if
	\pict{ContractionSPS1}
	is a \sps, then the \ps
	\pict{ContractionSPS2}
	is sequentializable (contraction).
\end{defn}

\begin{prop}[\cite{Girard:ProofNets}]
	\label{prop:Sequentialization}
	A \ps\ is sequentializable iff it is a \pn.
\end{prop}
The above result, combined with \refdef{SeqNet}, gives a simple intuition for looking at \pn s: they can be seen as a sort of ``graphical sequent calculus''.

\paragraph*{Cut-elimination.}
\begin{figure}[t]
	\pict{axstep}
	\caption{Axiom step.}
	\label{fig:AxStep}
\end{figure}
\begin{figure}[t]
	\pict{multstep}
	\caption{Multiplicative step.}
	\label{fig:MultStep}
\end{figure}
% \begin{figure}[pt]
% 	\pict{quantstep}
% 	\caption{Quantifier step; the substitution is performed on the whole net.}
% 	\label{fig:QuantStep}
% \end{figure}
\begin{figure}[t]
	\pict[0.7]{expstep}
	\caption{Exponential step; $\flat\Gamma$ is a multiset of \struct s, so one \paxl\ link, \whynot\ link, or wire in the picture may in some case stand for several (including zero) \paxl\ links, \whynot\ links, or wires.}
	\label{fig:ExpStep}
\end{figure}
Formulating the cut-elimination procedure in \pn s is quite simple: there are only three rules (or \emph{steps}, as we shall more often call them), taking the form of the graph-rewriting rules given in Figures~\ref{fig:AxStep} through~\ref{fig:ExpStep}. When a \pn\ $\pi$ is transformed into $\pi'$ by the application of one cut-elimination step, we write $\pi\betared\pi'$, and we say that $\pi$ \emph{$\beta$-reduces} to $\pi'$. Of course, in that case, if $\pi$ is a \pn, then $\pi'$ is also a \pn, i.e., cut-elimination preserves correctness.

% The following notions, taken from \cite{Tortora:AdditivesAndNormalizationI}, are needed to analyze the dynamics of \pn s under cut-elimination, and will prove to be quite useful in the sequel:
% \begin{defn}[Lift, residue]
% 	Whenever $\pi\onered\pi'$, by simple inspection of the cut-elimination rules it is clear that any link $l'$ of $\pi'$ different from a \cut\ comes from a unique (``the same'') link $l$ of $\pi$; we say that $l$ is the \emph{lift} of $l'$, and that $l'$ is a \emph{residue} of $l$. We define the lift and residues of a box in the same way.
% \end{defn}

\paragraph*{Untyped \pn s.}
It is also possible to consider an untyped version of \pn s:
\begin{defn}[Untyped \pn]
	\label{def:UProofNet}
	An untyped \pps\ is a directed graph with boxes built using the links of \reffig{Links} as in \refdef{Net}, but without any labels on edges, or any constraint induced by such labels. An untyped \ps\ is an untyped \pps\ such that:
	\begin{itemize}
		\item the conclusion of a \flatl\ link must be the premise of a \paxl\ or \whynot\ link;
		\item the premise of a \paxl\ link must be the conclusion of a \flatl\ or \paxl\ link, and the conclusion of \paxl\ link must be the premise of a \paxl\ or \whynot\ link;
		\item the premises of a \whynot\ link must be conclusions of \flatl\ or \pax\ links.
	\end{itemize}
	The notions of switching can be applied to untyped \pps s without any change, and hence the notion of correctness. We then define an untyped \pn\ as a correct untyped \ps.
\end{defn}

Observe that the cut-elimination steps of Figures~\ref{fig:AxStep}~through~\ref{fig:ExpStep} do not use formulas, i.e., they make sense also in an untyped framework. Therefore, cut-elimination can be defined also for untyped \pn s. Obviously, in the untyped case there may be ``clashes'', i.e., \cut\ links connecting the conclusions of two non-dual links. %In that case, the \cut\ link is said to be \emph{irreducible}; otherwise, we call it \emph{reducible}. Hence, untyped \pn s may admit normal forms which are not cut-free.

